Efficient Privacy-Preserving Machine Learning with Lightweight Trusted Hardware

In this paper, we propose a new secure machine learning inference platform assisted by a small dedicated security processor, which will be easier to protect and deploy compared to today's TEEs integrated into high-performance processors. Our platform provides three main advantages over the state-of-the-art: (i) We achieve significant performance improvements compared to state-of-the-art distributed Privacy-Preserving Machine Learning (PPML) protocols, with only a small security processor that is comparable to a discrete security chip such as the Trusted Platform Module (TPM) or on-chip security subsystems in SoCs similar to the Apple enclave processor. In the semi-honest setting with WAN/GPU, our scheme is 4X-63X faster than Falcon (PoPETs'21) and AriaNN (PoPETs'22) and 3.8X-12X more communication efficient. We achieve even higher performance improvements in the malicious setting. (ii) Our platform guarantees security with abort against malicious adversaries under honest majority assumption. (iii) Our technique is not limited by the size of secure memory in a TEE and can support high-capacity modern neural networks like ResNet18 and Transformer. While previous work investigated the use of high-performance TEEs in PPML, this work represents the first to show that even tiny secure hardware with really limited performance can be leveraged to significantly speed-up distributed PPML protocols if the protocol can be carefully designed for lightweight trusted hardware.

==> analysis.tex <==
\section{Theoretical Analysis}\label{sec:analysis}

In this section we provide a proof of the secrecy and also make an asymptotic cost analysis of \scheme.

\subsection{Security Analysis}\label{sec:proof}

To provide a security proof of \scheme, we construct our proof based on the real-world/ideal-world simulation paradigm \cite{goldreich2019play,canetti2000security,canetti2001universally} \ph{Don't make it too formally. Do not make it long when it's informal}. In an ideal world, the parties sends their inputs to a fully trusted third party which will evaluate the function for them faithfully. In the real world, however, the parties have to execute the protocols in the environment with the presence of adversaries. 

% We assume in an ideal world the parties complete the evaluation of a function by sending the data to a trusted party which computes the results correctly and will not leak any information. Such protocols they invoke are called the ideal functionalities. In a real world though, the parties execute our protocol with the presence of corrupted parties. 

To prove that a protocol is secure, the construction of a simulator for each adversary in the real world should be given. The simulator will simulate the view of other parties by answering their queries through calling the ideal functionalities. The proof is established by showing that the simulated views and the real views are indistinguishable
%. We'll show that our protocols are secure 
% \ph{mention that the comp power is bounded}
(i.e., the real and simulated views have exactly the same distribution ). The protocol does not guarantee the completion under a denial-of-service attack, but detects when integrity is broken due to malicious behaviours. Either case, the protocol simply resorts to aborting the computation.

Our definition of security is introduced in \autoref{sec:sm}. The protocol consists of multiple sub-protocols from \autoref{sec:protocol}. To prove the security of a protocol, we show that a simulator can simulate all interactions by calling the ideal functionality and provides the same distribution of the view. The security of the composed real protocol comes from the hybrid argument by defining a series of interactions $M_0,...M_k$ where $k$ is the total number of sub-protocols, $M_0$ is the real interaction and $M_k$ is the ideal interaction. For neighbored $M_i,M_{i+1}$, only the $i^{th}$ sub-protocol is replaced by its ideal functionalities, and are thus, indistinguishable from each other. Therefore, $M_0$ would be indistinguishable from $M_k$, which concludes our proof.

We assume, without loss of generality, that $P_2$ is corrupted. The ideal functionalities $\mathcal{F}_{\textsf{ReLU}}$, $\mathcal{F}_{\textsf{Maxpool}}$, $\mathcal{F}_{\textsf{BatchNorm}}$, $\mathcal{F}_{\textsf{LayerNorm}}$, $\mathcal{F}_{\textsf{Softmax}}$, $\mathcal{F}_{\textsf{MulReLU}}$ they are listed in \autoref{sec:idealf}. 
We skip the proof of $\Pi_{\textsf{init}}$ since the remote attestation and Diffie–Hellman key exchange are well established, and we refer the reader to previous work \cite{mohassel2018aby3, wagh2020falcon} for the proof of the basic protocols including $\Pi_{\textsf{Mul}},\Pi_{\textsf{MatMul}},\Pi_{\textsf{Reconst}}$ that we do not change \ph{phrase this}. Here we present the proof that $\Pi_{\textsf{ReLU}}$ is indeed secure:

\begin{theorem}
\autoref{p:relu} securely implements $\mathcal{F}_{\textsf{ReLU}}$ in semi-honest setting. \ph{Add the malicious setting one! The probability of party to injecting }
\end{theorem}

\ph{Simulator for Multiplication, Simulator for TEE}

\begin{proof}\label{proof:relu}
Since the {\LTEE}s have already acted as an ``ideal'' trusted functionality in the perspective of the parties, we can construct the simulator to generate the view of the adversaries simply by acting almost exactly as the trusted {\LTEE}. In $\Pi_{\textsf{ReLU}}$ of \autoref{p:relu}, without loss of generality assume $i=1$.

% If $P_1$ is corrupted, $\mathcal{F}_{\textsf{ReLU}}$

The simulator $\mathcal{S}$ do as follows: it outputs a uniformly random mask $\bmm\in\mathbb{Z}_L^n$ to $P_1$, then $P_1$ would compute and send $\bmx'_1 = \llb \bmx\rrb^L_1+\bmm\in\mathbb{Z}_L^n$ to $\mathcal{S}$. $\mathcal{S}$ will pass it to and $P_2$ will follow the protocol to send $\bmx'=\bmx'_1+\llb\bmx\rrb^L_{2}+\llb\bmx\rrb^L_{3}$ to $\mathcal{S}$. Now $\mathcal{S}$ will invoke $\mathcal{F}_{\textsf{ReLU}}$ and pass in an alternative RSS of $\bmx$: $(\bmx',-\bmm,\mathbf{0})$. The ideal function would return $\bmz=\textsf{ReLU}(\bmx)$ and $\bmb=\textsf{DReLU}(\bmx)$. Then $\mathcal{S}$ generates uniformly random shares of $\mathbf{0}$: $\llb \bmz^*\rrb^L\in\mathbb{Z}_L^n$ and $\llb \bmb^*\rrb^2\in\mathbb{Z}_2^n$, compute $\llb \bmz\rrb^L=((\llb \bmz^*\rrb^L_1+\bmz)_L,\llb \bmz^*\rrb^L_2,\llb \bmz^*\rrb^L_3)$ and $\llb \bmb^*\rrb^2=((\llb \bmb^*\rrb^2_1+\bmb)_2,\llb \bmb^*\rrb^2_2,\llb \bmb^*\rrb^2_3)$. Return $\llb \bmz\rrb^L_i,\llb \bmz\rrb^L_{i+1}$ and $\llb \bmb\rrb^2_i,\llb \bmb\rrb^2_{i+1}$ to $P_i$ respectively.

From the above realization we can observe that, the only difference between the transcripts of the above protocol and \autoref{p:relu} is that the distribution of all received values are uniformly random instead of pseudo-random. Due to the assumption of the pseudo-randomness, we cannot distinguish these two distribution, therefore the environment is unable to distinguish between the above two scenarios. This concludes the proof.

\end{proof}

Similar proof can be done for $\mathcal{F}_{\textsf{Maxpool}}$ , $\mathcal{F}_{\textsf{BatchNorm}}$, $\mathcal{F}_{\textsf{LayerNorm}}$, $\mathcal{F}_{\textsf{MulReLU}}$ as stated in \autoref{sec:expanse}. The corresponding simulators only need to change the ideal functionality they invoke and the mask generation accordingly. 



\begin{theorem}
\autoref{p:softmax} securely implements $\mathcal{F}_{\textsf{Softmax}}$ in semi-honest setting.
\end{theorem}

\begin{proof}
The proof follows exactly the same steps as the proof for $\Pi_{\textsf{ReLU}}$. The only difference is that two integers $m^*_i,q^*_i$ not in $\mathbb{Z}_{L}$ are masked and transmitted, instead of one which is in $\mathbb{Z}_{L}$.
Since $q^*_i\in\mathbb{Z}_{2^{33}}$, $m^*_i\in\mathbb{Z}_{2^{53}}$, any of the two values are distributed (pseudo) uniformly randomly in a larger finite field comparing to the normal shares which are in $\mathbb{Z}_{2^{32}}$. This already indicates they have $1/2^{33}$ or $1/2^{53}$ probability to be guessed by the receiver, or $1/2^{33}+1/2^{53}-1/2^{86}$ for either to be guessed, which are all less than the probability a regular share got guessed, $1/2^{32}$. Same or higher level of security is achieved in this case.

This proves the protocol is at lease as secure as $\Pi_{\textsf{ReLU}}$.

\end{proof}

% \ph{Thang plz check}

% \ed{I didn't try to fully follow the details of the proof. I'll trust Thang and Elaine for this part.}

\subsection{Analytical Cost Analysis}

% \ph{Compare with Falcon makes the table reasonable}

The cost analysis is shown in \autoref{tab:cost}. $n$ refers to total number of inputs (when batchsize is 1), $a,b,c$ refers to the matrix dimensions, $w,h$ refers to the filter size, $s$ refers to the total filter steps, $k$ refers to the bit size of the finite field and we count the exponent and mantissa part in \autoref{p:softmax} as $k$ and $2k$. Falcon \cite{wagh2020falcon} and AriaNN \cite{ryffel2020ariann} results are from their papers.
We see orders of magnitude of improvements in inter-party communication rounds comparing with Falcon, and significant theoretical communication amount reduction comparing with Both.

The actual speedup of a certain neural network depends on its structure including the proportion of non-linear layers, followup layers after linear layers (which benefits from \autoref{p:matmulrelu}), and the input dimensions, etc. The communication setting and computational power also matters, and we'll discuss further in \autoref{sec:experiment}.

% \begin{table*}[]

% \renewcommand\arraystretch{2}
%     \centering
%     \begin{tabularx}{\linewidth}{cccccccc }
   
%     \hline
%         \multirow{2}{*}{Protocol} &\multirow{2}{*}{Dependence}
%         &\multicolumn{2}{c}{Falcon Network}&\multicolumn{2}{c}{Our Network}
%         &\multicolumn{2}{c}{Our Chip}\\ \cline{3-8}
        
%         &  & Rounds&Comm& Rounds&Comm&Comm&No. of Mul\\\hline
        
%         \textsf{ReLU} & $n$ & $5+\log_2 l$ & $4kn$& 2 & $(k+1)n$ & $\frac{5(k+1)n}{3}$ & 0\\\hline
        
%         \textsf{MaxPool} & $m\tims m,\{w,h\},s$ &$(wh-1)(7+\log_2 l)$ & $5k+wh$ & 2 & $\frac{km^2+kwh+2(k+1)s}{3}$ & $\frac{2km^2+2kwh+3(k+1)s}{3}$ & 0\\\hline
        
%         \textsf{MatMul} with $f$ &  $(a\times b),(b\times c),\{w,h\},s$ &- & -& 2 &  $\frac{k(a\times c)+kwh+2(k+1)s}{3}$ & $\frac{2k(a\times c)+2kwh+3(k+1)s}{3}$ & 0\\\hline
        
%         \textsf{Softmax} & $n$ &-&-& 2 & $\frac{5kn}{3}$ & $\frac{11kn}{3}$ & $2n$ $^*$\\\hline
        
%         \textsf{BatchNorm/ LayerNorm} & $n$ &$15+5l+l\log_2 l$ &$kr+4krl+14krn$ & 2 & $kn$ & $\frac{4kn}{3}$ & $2n+1$\\
    
    
%     \hline
%     \end{tabularx}
%     \caption{Analytical Cost Analysis of Communication and computation cost with the chip \\$^*$: at most \ph{should I put it here? explain what is $l$,softmax?}}
%     \label{tab:cost}
% \end{table*}

\begin{table*}[]

\renewcommand\arraystretch{1.5}
    \centering
    \begin{tabular}{c|c|ccccc}
   
    \hline
        \textsf{Communication Type}&\textsf{Framework}& \textsf{ReLU} & \textsf{MaxPool}   &\textsf{BatchNorm/ LayerNorm}& \textsf{Softmax} 
        % &\textsf{MatMul} with $f$ 
        \\\hline
        \multirow{3}{*}{Network comm. rounds} 
        &Falcon+ &$10$           & $12(w^2-1)$            &335                &-
        % &-
        \\
        &AriaNN  &2              &3                      &9                  &-
        % &-
        \\
        &{\scheme} &2              &2                      &2                  &2
        % &-
        \\\hline
        \multirow{3}{*}{Network comm. data}  
        &Falcon+ &$16n$          & $20m^2+4w^2$           &$~224n$                &-
        % &-
        \\
        &AriaNN  &$12n$          &$((m-w)/s+1)^2(w^4+1)$ &$72n$                  &-
        % &-
        \\
        &{\scheme} &$5n$           &$\frac{2}{3}(2n+2w^2+5((m-w)/s+1)^2)$ &$4n$  
                                &$\frac{20}{3}n$   
        % &$\frac{1}{3}(4(a\times c)+4w^2+10((m-w)/s+1)^2$    
        \\\hline
        \LTEE comm.  &{\scheme} &$\frac{25}{3}n$     &$\frac{1}{3}(8m^2+8w^2+15((m-w)/s+1)^2)$    &$\frac{16}{3}n$ &$\frac{44}{3}n$\\
        
    
    \hline
    \end{tabular}
    \caption{Analytical cost analysis of the network communication rounds and amount (in MB), and the local bus communication with the LEE. Here $n=m\times m$ is the input size, $s$ is stride and the filter size is set to be $w\times w$.}
    \label{tab:cost}
\end{table*}

==> fig/main_results.tex <==

\begin{table*}[ht]

\renewcommand\arraystretch{0.9}
    \centering
    % \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{x{1.8cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}}
    % {\linewidth}{c|cccc|cccc|cccc}
    \hline
        &  \multicolumn{4}{c|}{Network-A} &\multicolumn{4}{c|}{Network-B}
        &\multicolumn{4}{c}{Network-C}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        
        Falcon+ &0.0824&0.1118&1.478&1.393&0.2034&0.2618&1.464&1.292&1.866&2.191&7.321&7.288\\
        AriaNN &0.2560 &0.5120 &-     &5.504 &-     &-     &-     &-  &3.072 &5.248 &-     &17.02   \\
        \scheme-chip    &\textbf{0.0737}&\textbf{0.0777}&\textbf{0.2516}&\textbf{0.2946}&\textbf{0.1172}&\textbf{0.1142}&\textbf{0.2787}&\textbf{0.2938}&\textbf{0.6809}&\textbf{1.298}&\textbf{1.024}&\textbf{1.494}\\
       speed-up & 1.11$\times$ &{ 1.43$\times$ }&{ 5.87$\times$ }&{ 4.72$\times$ }&{ 1.73$\times$ }&{ 2.29$\times$ }&{5.25$\times$ }&{ 4.39$\times$ }&{ 2.74$\times$ }&{ 1.68$\times$ }&{ 7.14$\times$ }& {4.87$\times$}\\\hline
        \scheme-SoC    &0.0432	&0.0472	&0.2211	&0.2641	&0.0643	&0.0613	&0.1994	&0.2408 &0.1990	&0.8163	&0.5424	&1.012\\
         speed-up &1.91$\times$	& 2.37$\times$	& 6.69$\times$	& 5.28$\times$	&    3.17$\times$	& 4.28$\times$	& 7.34$\times$	& 5.37$\times$	&    9.38$\times$	& 3.10$\times$	& 13.5$\times$	& 7.20$\times$	   \\\hline
    \hline
        &\multicolumn{4}{c|}{LeNet}&\multicolumn{4}{c|}{AlexNet}&\multicolumn{4}{c}{Transformer}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        Falcon+ &2.592&4.603&8.867&9.563&4.276&11.78&38.56&43.06&4.026&-&321.0&-
        \\
        AriaNN &4.480 &7.040 &-     &18.30&9.984&19.20&-&43.52  &-&-&-& -     \\
        \scheme-chip    &\textbf{0.9693}&\textbf{3.075}&\textbf{1.315}&\textbf{3.255
        }&\textbf{1.564}&\textbf{9.263}&\textbf{2.463}&\textbf{9.449}&\textbf{0.5130}&-&\textbf{5.024}&-\\
        
        speed-up    & 2.67$\times$ & 1.49$\times$ & 6.74$\times$ & 2.93$\times$ & 2.73$\times$ & 1.27$\times$ & 15.6$\times$ & 4.55$\times$ & 7.84$\times$ & - & 63.8$\times$ &-\\\hline
        \scheme-SoC &0.2869	&2.392	&0.6328	&2.573 &0.3055	&8.029	&1.229	&8.215 &0.3618	&-	&4.873	&-\\
        speed-up   & 9.04$\times$	& 2.02$\times$	& 14.0$\times$	& 3.72$\times$	&    14.0$\times$	& 1.52$\times$	& 31.3$\times$	& 5.24$\times$	&   11.1$\times$	&-	& 65.8$\times$	&-
        \\\hline
    \hline
        &\multicolumn{4}{c|}{VGG16}&\multicolumn{4}{c|}{ResNet18}&\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\cline{0-8}
        Falcon+ &49.36&-&122.1&-&545.9&-&1439&\\
        AriaNN* &198.4&-&-&-&1779&-&-&-        \\
        \scheme-chip    &\textbf{26.55}&-&\textbf{30.05}&-&\textbf{309.7}&-&\textbf{350.7}&-\\
       
        speed-up    &1.85$\times$&-&4.06$\times$&-&1.76$\times$&-&4.10$\times$&-\\
    \cline{0-8}
    \scheme-SoC & 13.06	&-	&16.56	&- &106.9	&-	&148.0	&-\\
    speed-up   &3.78$\times$	&-	&7.37$\times$	&-    &5.10$\times$	&-	&9.72$\times$	&-
        \\\hline\hline
    \end{tabular}
% 	\end{adjustbox}

    \caption{Inference time (s) of a 128 batch in a semi-honest setting. AriaNN has a reduced batch size of 64 and 8 for VGG16 and ResNet18 due to memory consumption, which also applies to other tables.}
    \label{tab:time_semi}
\end{table*}

\begin{table*}[ht]

\renewcommand\arraystretch{0.9}
    \centering
    
    \begin{tabular}{x{1.8cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}}
    \hline
    \hline
        &  \multicolumn{4}{c|}{Network-A} &\multicolumn{4}{c|}{Network-B}
        &\multicolumn{4}{c}{Network-C}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        
        Falcon+ &0.1921&0.3293&3.359&3.3701&0.6279&0.6416&3.504&3.0743&5.639&6.758&23.26&20.8988
\\
        \scheme-chip    &\textbf{0.0913}&\textbf{0.2567}&\textbf{0.5150}&\textbf{0.7307}&\textbf{0.1594}&\textbf{0.2860}&\textbf{0.5803}&\textbf{0.7246}&\textbf{1.157}&\textbf{3.661}&\textbf{2.196}&\textbf{4.258}\\

        speed-up    &2.10$\times$&1.51$\times$&6.52$\times$&4.61$\times$&3.94$\times$&2.82$\times$&6.04$\times$&4.24$\times$&4.87$\times$&2.12$\times$&10.6$\times$&4.91$\times$
\\\hline
        \scheme-SoC &0.0200	&0.1854	&0.4437	&0.6594  &0.0357	&0.1623	&0.4566	&0.6010 &0.0325	&2.536	&1.071	&3.134\\
        speed-up   &9.59$\times$	&2.09$\times$	&7.57$\times$	&5.11$\times$	&    17.5$\times$	&4.98$\times$	&7.67$\times$	&5.12$\times$	&    173$\times$	&3.06$\times$	&21.7$\times$	&6.67$\times$	
        \\\hline
    \hline
        &\multicolumn{4}{c|}{LeNet}&\multicolumn{4}{c|}{AlexNet}&\multicolumn{4}{c}{Transformer}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        Falcon+ &7.492&15.38&28.82&32.57&13.89&41.88&100.9&123.2&10.99&-&777.9&-\\
        \scheme-chip    &\textbf{2.106}&\textbf{10.64}&\textbf{2.929}&\textbf{10.80}&\textbf{3.653}&\textbf{36.80}&\textbf{5.538}&\textbf{36.10}&\textbf{2.073}&-&\textbf{13.03}&-\\
        speed-up    &3.56$\times$&1.55$\times$&9.84$\times$&3.01$\times$&3.80$\times$&1.27$\times$&18.2$\times$&3.41$\times$&5.30$\times$&-&59.6$\times$&-\\\hline
        \scheme-SoC    &0.5136	&9.052	&1.337	&9.213  &0.7738	&33.92	&2.659	&33.22    &1.720	&-	&12.68	&-\\
        speed-up   &14.5$\times$	&1.82$\times$	&21.5$\times$	&3.54$\times$	&    17.9$\times$	&1.37$\times$	&37.9$\times$	&3.71$\times$	&    6.39$\times$	&-	&61.3$\times$	&-
        \\\hline\hline

        &\multicolumn{4}{c|}{VGG16}&\multicolumn{4}{c|}{ResNet18}&\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\cline{0-8}
        Falcon+ &136.9&-&407.8&-&1550&-&4993&-\\
        \scheme-chip    &\textbf{51.54}&-&\textbf{68.09}&-&\textbf{639.3}&-&\textbf{772.2}&-\\
        speed-up    &2.66$\times$&-&5.99$\times$&-&2.43$\times$&-&6.47$\times$&-\\\cline{0-8}
        \scheme-SoC &20.06	&-	&36.62	&-  &166.2	&-	&299.1	&-\\
        speed-up   &6.82$\times$	&-	&11.1$\times$	&-    &9.33$\times$	&-	&16.6$\times$	&-   
        \\\hline
    \hline
    \end{tabular}


    \caption{Inference time (s) of a 128 batch in a malicious setting. AriaNN does not implement their work in a malicious setting.}
    \label{tab:time_mal}
\end{table*}

\begin{table*}[ht]

% \renewcommand\arraystretch{1}
    \centering

    \begin{tabular}{cc|cccccccc}
    \hline
    
        \multicolumn{2}{c|}{Framework} &  Network-A    &Network-B  &Network-C  &LeNet  &AlexNet    &Transformer    &VGG16 &ResNet18 \\\hline
        
        Falcon+ &Inter-party    &1.536  &6.272 &64.87  &95.33    &173.5    &72.21    &1730 &22933\\\hline

        AriaNN  &Inter-party      &2.816  &  - &38.54      &55.04     &121.6      &-      &1161    &18944\\\hline
        \multirow{2}{*}{\scheme}    &Inter-party    &0.2058	&0.8371	&5.328	&7.931	&12.31	    &19.21 &187.7	&2106	\\\cline{2-10}
        &\LTH-CPU &0.4585	    &0.7958	    &7.235&10.24	&18.53	&2.270   &202.5	&3044	

        \\\hline
    
    \end{tabular}


    \caption{Inference communication(MB) of a 128 batch in a semi-honest setting.}
    \label{tab:comm_sem}
\end{table*}

\begin{table*}[ht]

\renewcommand\arraystretch{1}
    \centering

    \begin{tabular}{cc|cccccccc}
    \hline
    
        \multicolumn{2}{c|}{Framework} &  Network-A    &Network-B  &Network-C  &LeNet  &AlexNet    &Transformer    &VGG16 &ResNet18 \\\hline
        
        Falcon+     &Inter-party    &10.51     &41.33     &423.4&620.1    &1135    &340.0    &11543&139287\\\hline
        \multirow{2}{*}{\scheme}    &Inter-party        &0.8443     &2.0704	    &21.02&28.80    &48.68	&131.2     &838.6	&7500	\\
    \cline{2-10}
        &\LTH-CPU &1.070	&1.856	&16.88	&23.90	&43.23&5.296	&472.5	&7103


        \\\hline
    
    \end{tabular}


    \caption{Inference communication (MB) of a 128 batch in a malicious setting.}
    \label{tab:comm_mal}
\end{table*}

\begin{table*}[ht]
% \renewcommand\arraystretch{1.2}
\setlength\tabcolsep{3pt}
    \centering

    \begin{tabular}{x{1.5cm}x{1.8cm}|x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.7cm}x{0.7cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}}
    \hline
        \multirow{2}{*}{Framework}&  \multirow{2}{*}{Component}&  \multicolumn{2}{c}{Network-A}    &\multicolumn{2}{c}{Network-B} &\multicolumn{2}{c}{Network-C}  &\multicolumn{2}{c}{LeNet} &\multicolumn{2}{c}{AlexNet}   &\multicolumn{2}{c}{Transformer}    &\multicolumn{2}{c}{VGG16}     &\multicolumn{2}{c}{ResNet18} \\
        && Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio\\ \hline
        \multirow{3}{*}{\scheme} &CPU/GPU &0.04  & 17\%  & 0.06  & 23\%  & 0.19  & 19\%  & 0.28  & 21\%  & 0.29  & 12\%  & 0.30  & 6\%  & 12.8  & 43\%  & 98.0 & 28\%  \\ 
       & Comm. &0.18  & 70\%  & 0.16  & 58\%  & 0.35  & 34\%  & 0.35  & 27\%  & 0.94  & 38\%  & 4.56  & 91\%  & 3.34  & 11\%  & 44.0 & 13\%  \\ 
       & LTH &0.03  & 13\%  & 0.05  & 19\%  & 0.48  & 47\%  & 0.68  & 52\%  & 1.24  & 50\%  & 0.16  & 3\%  & 13.8  & 46\%  & 207 & 59\%  \\ \hline
        \multirow{2}{*}{Falcon+} &CPU/GPU &0.08  & 6\%  & 0.20  & 14\%  & 1.80  & 25\%  & 2.50  & 28\%  & 4.09  & 11\%  & 3.95  & 1\%  & 47.6  & 39\%  & 523 & 36\%  \\ 
        &Comm. &1.40  & 94\%  & 1.27  & 86\%  & 5.52  & 75\%  & 6.37  & 72\%  & 34.4  & 89\%  & 317  & 99\%  & 74.4  & 61\%  & 916 & 64\%  \\\hline
    \end{tabular}
	

    
    \caption{Inference time (s) breakdown of a 128 batch in a semi-honest WAN/GPU setting, comparing with Falcon+.}
    \label{tab:breakdown}
\end{table*}

==> main_results.tex <==

\begin{table*}[ht]

\renewcommand\arraystretch{0.9}
    \centering
    % \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{x{1.8cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}}
    % {\linewidth}{c|cccc|cccc|cccc}
    \hline
        &  \multicolumn{4}{c|}{Network-A} &\multicolumn{4}{c|}{Network-B}
        &\multicolumn{4}{c}{Network-C}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        
        Falcon+ &0.0824&0.1118&1.478&1.393&0.2034&0.2618&1.464&1.292&1.866&2.191&7.321&7.288\\
        AriaNN &0.2560 &0.5120 &-     &5.504 &-     &-     &-     &-  &3.072 &5.248 &-     &17.02   \\
        \scheme-chip    &\textbf{0.0737}&\textbf{0.0777}&\textbf{0.2516}&\textbf{0.2946}&\textbf{0.1172}&\textbf{0.1142}&\textbf{0.2787}&\textbf{0.2938}&\textbf{0.6809}&\textbf{1.298}&\textbf{1.024}&\textbf{1.494}\\
       speed-up & 1.11$\times$ &{ 1.43$\times$ }&{ 5.87$\times$ }&{ 4.72$\times$ }&{ 1.73$\times$ }&{ 2.29$\times$ }&{5.25$\times$ }&{ 4.39$\times$ }&{ 2.74$\times$ }&{ 1.68$\times$ }&{ 7.14$\times$ }& {4.87$\times$}\\\hline
        \scheme-SoC    &0.0432	&0.0472	&0.2211	&0.2641	&0.0643	&0.0613	&0.1994	&0.2408 &0.1990	&0.8163	&0.5424	&1.012\\
         speed-up &1.91$\times$	& 2.37$\times$	& 6.69$\times$	& 5.28$\times$	&    3.17$\times$	& 4.28$\times$	& 7.34$\times$	& 5.37$\times$	&    9.38$\times$	& 3.10$\times$	& 13.5$\times$	& 7.20$\times$	   \\\hline
    \hline
        &\multicolumn{4}{c|}{LeNet}&\multicolumn{4}{c|}{AlexNet}&\multicolumn{4}{c}{Transformer}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        Falcon+ &2.592&4.603&8.867&9.563&4.276&11.78&38.56&43.06&4.026&-&321.0&-
        \\
        AriaNN &4.480 &7.040 &-     &18.30&9.984&19.20&-&43.52  &-&-&-& -     \\
        \scheme-chip    &\textbf{0.9693}&\textbf{3.075}&\textbf{1.315}&\textbf{3.255
        }&\textbf{1.564}&\textbf{9.263}&\textbf{2.463}&\textbf{9.449}&\textbf{0.5130}&-&\textbf{5.024}&-\\
        
        speed-up    & 2.67$\times$ & 1.49$\times$ & 6.74$\times$ & 2.93$\times$ & 2.73$\times$ & 1.27$\times$ & 15.6$\times$ & 4.55$\times$ & 7.84$\times$ & - & 63.8$\times$ &-\\\hline
        \scheme-SoC &0.2869	&2.392	&0.6328	&2.573 &0.3055	&8.029	&1.229	&8.215 &0.3618	&-	&4.873	&-\\
        speed-up   & 9.04$\times$	& 2.02$\times$	& 14.0$\times$	& 3.72$\times$	&    14.0$\times$	& 1.52$\times$	& 31.3$\times$	& 5.24$\times$	&   11.1$\times$	&-	& 65.8$\times$	&-
        \\\hline
    \hline
        &\multicolumn{4}{c|}{VGG16}&\multicolumn{4}{c|}{ResNet18}&\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\cline{0-8}
        Falcon+ &49.36&-&122.1&-&545.9&-&1439&\\
        AriaNN* &198.4&-&-&-&1779&-&-&-        \\
        \scheme-chip    &\textbf{26.55}&-&\textbf{30.05}&-&\textbf{309.7}&-&\textbf{350.7}&-\\
       
        speed-up    &1.85$\times$&-&4.06$\times$&-&1.76$\times$&-&4.10$\times$&-\\
    \cline{0-8}
    \scheme-SoC & 13.06	&-	&16.56	&- &106.9	&-	&148.0	&-\\
    speed-up   &3.78$\times$	&-	&7.37$\times$	&-    &5.10$\times$	&-	&9.72$\times$	&-
        \\\hline\hline
    \end{tabular}
% 	\end{adjustbox}

    \caption{Inference time (s) of a 128 batch in a semi-honest setting. AriaNN has a reduced batch size of 64 and 8 for VGG16 and ResNet18 due to memory consumption, which also applies to other tables.}
    \label{tab:time_semi}
\end{table*}

\begin{table*}[ht]

\renewcommand\arraystretch{0.9}
    \centering
    
    \begin{tabular}{x{1.8cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}}
    \hline
    \hline
        &  \multicolumn{4}{c|}{Network-A} &\multicolumn{4}{c|}{Network-B}
        &\multicolumn{4}{c}{Network-C}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        
        Falcon+ &0.1921&0.3293&3.359&3.3701&0.6279&0.6416&3.504&3.0743&5.639&6.758&23.26&20.8988
\\
        \scheme-chip    &\textbf{0.0913}&\textbf{0.2567}&\textbf{0.5150}&\textbf{0.7307}&\textbf{0.1594}&\textbf{0.2860}&\textbf{0.5803}&\textbf{0.7246}&\textbf{1.157}&\textbf{3.661}&\textbf{2.196}&\textbf{4.258}\\

        speed-up    &2.10$\times$&1.51$\times$&6.52$\times$&4.61$\times$&3.94$\times$&2.82$\times$&6.04$\times$&4.24$\times$&4.87$\times$&2.12$\times$&10.6$\times$&4.91$\times$
\\\hline
        \scheme-SoC &0.0200	&0.1854	&0.4437	&0.6594  &0.0357	&0.1623	&0.4566	&0.6010 &0.0325	&2.536	&1.071	&3.134\\
        speed-up   &9.59$\times$	&2.09$\times$	&7.57$\times$	&5.11$\times$	&    17.5$\times$	&4.98$\times$	&7.67$\times$	&5.12$\times$	&    173$\times$	&3.06$\times$	&21.7$\times$	&6.67$\times$	
        \\\hline
    \hline
        &\multicolumn{4}{c|}{LeNet}&\multicolumn{4}{c|}{AlexNet}&\multicolumn{4}{c}{Transformer}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        Falcon+ &7.492&15.38&28.82&32.57&13.89&41.88&100.9&123.2&10.99&-&777.9&-\\
        \scheme-chip    &\textbf{2.106}&\textbf{10.64}&\textbf{2.929}&\textbf{10.80}&\textbf{3.653}&\textbf{36.80}&\textbf{5.538}&\textbf{36.10}&\textbf{2.073}&-&\textbf{13.03}&-\\
        speed-up    &3.56$\times$&1.55$\times$&9.84$\times$&3.01$\times$&3.80$\times$&1.27$\times$&18.2$\times$&3.41$\times$&5.30$\times$&-&59.6$\times$&-\\\hline
        \scheme-SoC    &0.5136	&9.052	&1.337	&9.213  &0.7738	&33.92	&2.659	&33.22    &1.720	&-	&12.68	&-\\
        speed-up   &14.5$\times$	&1.82$\times$	&21.5$\times$	&3.54$\times$	&    17.9$\times$	&1.37$\times$	&37.9$\times$	&3.71$\times$	&    6.39$\times$	&-	&61.3$\times$	&-
        \\\hline\hline

        &\multicolumn{4}{c|}{VGG16}&\multicolumn{4}{c|}{ResNet18}&\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\cline{0-8}
        Falcon+ &136.9&-&407.8&-&1550&-&4993&-\\
        \scheme-chip    &\textbf{51.54}&-&\textbf{68.09}&-&\textbf{639.3}&-&\textbf{772.2}&-\\
        speed-up    &2.66$\times$&-&5.99$\times$&-&2.43$\times$&-&6.47$\times$&-\\\cline{0-8}
        \scheme-SoC &20.06	&-	&36.62	&-  &166.2	&-	&299.1	&-\\
        speed-up   &6.82$\times$	&-	&11.1$\times$	&-    &9.33$\times$	&-	&16.6$\times$	&-   
        \\\hline
    \hline
    \end{tabular}


    \caption{Inference time (s) of a 128 batch in a malicious setting. AriaNN does not implement their work in a malicious setting.}
    \label{tab:time_mal}
\end{table*}

\begin{table*}[ht]

% \renewcommand\arraystretch{1}
    \centering

    \begin{tabular}{cc|cccccccc}
    \hline
    
        \multicolumn{2}{c|}{Framework} &  Network-A    &Network-B  &Network-C  &LeNet  &AlexNet    &Transformer    &VGG16 &ResNet18 \\\hline
        
        Falcon+ &Inter-party    &1.536  &6.272 &64.87  &95.33    &173.5    &72.21    &1730 &22933\\\hline

        AriaNN  &Inter-party      &2.816  &  - &38.54      &55.04     &121.6      &-      &1161    &18944\\\hline
        \multirow{2}{*}{\scheme}    &Inter-party    &0.2058	&0.8371	&5.328	&7.931	&12.31	    &19.21 &187.7	&2106	\\\cline{2-10}
        &\LTH-CPU &0.4585	    &0.7958	    &7.235&10.24	&18.53	&2.270   &202.5	&3044	

        \\\hline
    
    \end{tabular}


    \caption{Inference communication(MB) of a 128 batch in a semi-honest setting.}
    \label{tab:comm_sem}
\end{table*}

\begin{table*}[ht]

\renewcommand\arraystretch{1}
    \centering

    \begin{tabular}{cc|cccccccc}
    \hline
    
        \multicolumn{2}{c|}{Framework} &  Network-A    &Network-B  &Network-C  &LeNet  &AlexNet    &Transformer    &VGG16 &ResNet18 \\\hline
        
        Falcon+     &Inter-party    &10.51     &41.33     &423.4&620.1    &1135    &340.0    &11543&139287\\\hline
        \multirow{2}{*}{\scheme}    &Inter-party        &0.8443     &2.0704	    &21.02&28.80    &48.68	&131.2     &838.6	&7500	\\
    \cline{2-10}
        &\LTH-CPU &1.070	&1.856	&16.88	&23.90	&43.23&5.296	&472.5	&7103


        \\\hline
    
    \end{tabular}


    \caption{Inference communication (MB) of a 128 batch in a malicious setting.}
    \label{tab:comm_mal}
\end{table*}

\begin{table*}[ht]
% \renewcommand\arraystretch{1.2}
\setlength\tabcolsep{3pt}
    \centering

    \begin{tabular}{x{1.5cm}x{1.8cm}|x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.7cm}x{0.7cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}}
    \hline
        \multirow{2}{*}{Framework}&  \multirow{2}{*}{Component}&  \multicolumn{2}{c}{Network-A}    &\multicolumn{2}{c}{Network-B} &\multicolumn{2}{c}{Network-C}  &\multicolumn{2}{c}{LeNet} &\multicolumn{2}{c}{AlexNet}   &\multicolumn{2}{c}{Transformer}    &\multicolumn{2}{c}{VGG16}     &\multicolumn{2}{c}{ResNet18} \\
        && Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio\\ \hline
        \multirow{3}{*}{\scheme} &CPU/GPU &0.04  & 17\%  & 0.06  & 23\%  & 0.19  & 19\%  & 0.28  & 21\%  & 0.29  & 12\%  & 0.30  & 6\%  & 12.8  & 43\%  & 98.0 & 28\%  \\ 
       & Comm. &0.18  & 70\%  & 0.16  & 58\%  & 0.35  & 34\%  & 0.35  & 27\%  & 0.94  & 38\%  & 4.56  & 91\%  & 3.34  & 11\%  & 44.0 & 13\%  \\ 
       & LTH &0.03  & 13\%  & 0.05  & 19\%  & 0.48  & 47\%  & 0.68  & 52\%  & 1.24  & 50\%  & 0.16  & 3\%  & 13.8  & 46\%  & 207 & 59\%  \\ \hline
        \multirow{2}{*}{Falcon+} &CPU/GPU &0.08  & 6\%  & 0.20  & 14\%  & 1.80  & 25\%  & 2.50  & 28\%  & 4.09  & 11\%  & 3.95  & 1\%  & 47.6  & 39\%  & 523 & 36\%  \\ 
        &Comm. &1.40  & 94\%  & 1.27  & 86\%  & 5.52  & 75\%  & 6.37  & 72\%  & 34.4  & 89\%  & 317  & 99\%  & 74.4  & 61\%  & 916 & 64\%  \\\hline
    \end{tabular}
	

    
    \caption{Inference time (s) breakdown of a 128 batch in a semi-honest WAN/GPU setting, comparing with Falcon+.}
    \label{tab:breakdown}
\end{table*}

==> table1.tex <==
\begin{table*}[ht]
\small 
\renewcommand\arraystretch{0.9}
    \centering
    % \begin{adjustbox}{width=\textwidth}
    \caption{Inference time (s) of a 128 batch in a semi-honest setting. AriaNN has a reduced batch size of 64 and 8 for VGG16 and ResNet18 due to memory consumption, which also applies to other tables.}
    \begin{tabular}{x{1.8cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}}
    % {\linewidth}{c|cccc|cccc|cccc}
    \hline
        &  \multicolumn{4}{c|}{Network-A} &\multicolumn{4}{c|}{Network-B}
        &\multicolumn{4}{c}{Network-C}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        
        Falcon+ &0.0824&0.1118&1.478&1.393&0.2034&0.2618&1.464&1.292&1.866&2.191&7.321&7.288\\
        AriaNN &0.2560 &0.5120 &-     &5.504 &-     &-     &-     &-  &3.072 &5.248 &-     &17.02   \\
        \scheme-chip    &\textbf{0.0737}&\textbf{0.0777}&\textbf{0.2516}&\textbf{0.2946}&\textbf{0.1172}&\textbf{0.1142}&\textbf{0.2787}&\textbf{0.2938}&\textbf{0.6809}&\textbf{1.298}&\textbf{1.024}&\textbf{1.494}\\
       speed-up & 1.11$\times$ &{ 1.43$\times$ }&{ 5.87$\times$ }&{ 4.72$\times$ }&{ 1.73$\times$ }&{ 2.29$\times$ }&{5.25$\times$ }&{ 4.39$\times$ }&{ 2.74$\times$ }&{ 1.68$\times$ }&{ 7.14$\times$ }& {4.87$\times$}\\\hline
        \scheme-SoC    &0.0432	&0.0472	&0.2211	&0.2641	&0.0643	&0.0613	&0.1994	&0.2408 &0.1990	&0.8163	&0.5424	&1.012\\
         speed-up &1.91$\times$	& 2.37$\times$	& 6.69$\times$	& 5.28$\times$	&    3.17$\times$	& 4.28$\times$	& 7.34$\times$	& 5.37$\times$	&    9.38$\times$	& 3.10$\times$	& 13.5$\times$	& 7.20$\times$	   \\\hline
    \hline
        &\multicolumn{4}{c|}{LeNet}&\multicolumn{4}{c|}{AlexNet}&\multicolumn{4}{c}{Transformer}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        Falcon+ &2.592&4.603&8.867&9.563&4.276&11.78&38.56&43.06&4.026&-&321.0&-
        \\
        AriaNN &4.480 &7.040 &-     &18.30&9.984&19.20&-&43.52  &-&-&-& -     \\
        \scheme-chip    &\textbf{0.9693}&\textbf{3.075}&\textbf{1.315}&\textbf{3.255
        }&\textbf{1.564}&\textbf{9.263}&\textbf{2.463}&\textbf{9.449}&\textbf{0.5130}&-&\textbf{5.024}&-\\
        
        speed-up    & 2.67$\times$ & 1.49$\times$ & 6.74$\times$ & 2.93$\times$ & 2.73$\times$ & 1.27$\times$ & 15.6$\times$ & 4.55$\times$ & 7.84$\times$ & - & 63.8$\times$ &-\\\hline
        \scheme-SoC &0.2869	&2.392	&0.6328	&2.573 &0.3055	&8.029	&1.229	&8.215 &0.3618	&-	&4.873	&-\\
        speed-up   & 9.04$\times$	& 2.02$\times$	& 14.0$\times$	& 3.72$\times$	&    14.0$\times$	& 1.52$\times$	& 31.3$\times$	& 5.24$\times$	&   11.1$\times$	&-	& 65.8$\times$	&-
        \\\hline
    \hline
        &\multicolumn{4}{c|}{VGG16}&\multicolumn{4}{c|}{ResNet18}&\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\cline{0-8}
        Falcon+ &49.36&-&122.1&-&545.9&-&1439&\\
        AriaNN* &198.4&-&-&-&1779&-&-&-        \\
        \scheme-chip    &\textbf{26.55}&-&\textbf{30.05}&-&\textbf{309.7}&-&\textbf{350.7}&-\\
       
        speed-up    &1.85$\times$&-&4.06$\times$&-&1.76$\times$&-&4.10$\times$&-\\
    \cline{0-8}
    \scheme-SoC & 13.06	&-	&16.56	&- &106.9	&-	&148.0	&-\\
    speed-up   &3.78$\times$	&-	&7.37$\times$	&-    &5.10$\times$	&-	&9.72$\times$	&-
        \\\hline\hline
    \end{tabular}
% 	\end{adjustbox}

    
    \label{tab:time_semi}
\end{table*}


==> table2.tex <==
\begin{table*}[ht]
\small 
\renewcommand\arraystretch{0.9}
    \centering
    \caption{Inference time (s) of a 128 batch in a malicious setting. AriaNN does not implement their work in a malicious setting.}
    \begin{tabular}{x{1.8cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}|x{0.86cm}x{0.86cm}x{0.86cm}x{0.86cm}}
    \hline
    \hline
    
        &  \multicolumn{4}{c|}{Network-A} &\multicolumn{4}{c|}{Network-B}
        &\multicolumn{4}{c}{Network-C}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        
        Falcon+ &0.1921&0.3293&3.359&3.3701&0.6279&0.6416&3.504&3.0743&5.639&6.758&23.26&20.8988
\\
        \scheme-chip    &\textbf{0.0913}&\textbf{0.2567}&\textbf{0.5150}&\textbf{0.7307}&\textbf{0.1594}&\textbf{0.2860}&\textbf{0.5803}&\textbf{0.7246}&\textbf{1.157}&\textbf{3.661}&\textbf{2.196}&\textbf{4.258}\\

        speed-up    &2.10$\times$&1.51$\times$&6.52$\times$&4.61$\times$&3.94$\times$&2.82$\times$&6.04$\times$&4.24$\times$&4.87$\times$&2.12$\times$&10.6$\times$&4.91$\times$
\\\hline
        \scheme-SoC &0.0200	&0.1854	&0.4437	&0.6594  &0.0357	&0.1623	&0.4566	&0.6010 &0.0325	&2.536	&1.071	&3.134\\
        speed-up   &9.59$\times$	&2.09$\times$	&7.57$\times$	&5.11$\times$	&    17.5$\times$	&4.98$\times$	&7.67$\times$	&5.12$\times$	&    173$\times$	&3.06$\times$	&21.7$\times$	&6.67$\times$	
        \\\hline
    \hline
        &\multicolumn{4}{c|}{LeNet}&\multicolumn{4}{c|}{AlexNet}&\multicolumn{4}{c}{Transformer}\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\hline
        Falcon+ &7.492&15.38&28.82&32.57&13.89&41.88&100.9&123.2&10.99&-&777.9&-\\
        \scheme-chip    &\textbf{2.106}&\textbf{10.64}&\textbf{2.929}&\textbf{10.80}&\textbf{3.653}&\textbf{36.80}&\textbf{5.538}&\textbf{36.10}&\textbf{2.073}&-&\textbf{13.03}&-\\
        speed-up    &3.56$\times$&1.55$\times$&9.84$\times$&3.01$\times$&3.80$\times$&1.27$\times$&18.2$\times$&3.41$\times$&5.30$\times$&-&59.6$\times$&-\\\hline
        \scheme-SoC    &0.5136	&9.052	&1.337	&9.213  &0.7738	&33.92	&2.659	&33.22    &1.720	&-	&12.68	&-\\
        speed-up   &14.5$\times$	&1.82$\times$	&21.5$\times$	&3.54$\times$	&    17.9$\times$	&1.37$\times$	&37.9$\times$	&3.71$\times$	&    6.39$\times$	&-	&61.3$\times$	&-
        \\\hline\hline

        &\multicolumn{4}{c|}{VGG16}&\multicolumn{4}{c|}{ResNet18}&\\
        &  LAN & LAN &WAN &WAN & LAN & LAN &WAN &WAN & \\
        Framework&  GPU & CPU &GPU &CPU & GPU & CPU &GPU &CPU \\\cline{0-8}
        Falcon+ &136.9&-&407.8&-&1550&-&4993&-\\
        \scheme-chip    &\textbf{51.54}&-&\textbf{68.09}&-&\textbf{639.3}&-&\textbf{772.2}&-\\
        speed-up    &2.66$\times$&-&5.99$\times$&-&2.43$\times$&-&6.47$\times$&-\\\cline{0-8}
        \scheme-SoC &20.06	&-	&36.62	&-  &166.2	&-	&299.1	&-\\
        speed-up   &6.82$\times$	&-	&11.1$\times$	&-    &9.33$\times$	&-	&16.6$\times$	&-   
        \\\hline
    \hline
    \end{tabular}


    
    \label{tab:time_mal}
\end{table*}

==> table3.tex <==
\begin{table*}[ht]
\small 
% \renewcommand\arraystretch{1}
    \centering
    \caption{Inference communication(MB) of a 128 batch in a semi-honest setting.}
    \begin{tabular}{cc|cccccccc}
    \hline
    
        \multicolumn{2}{c|}{Framework} &  Network-A    &Network-B  &Network-C  &LeNet  &AlexNet    &Transformer    &VGG16 &ResNet18 \\\hline
        
        Falcon+ &Inter-party    &1.536  &6.272 &64.87  &95.33    &173.5    &72.21    &1730 &22933\\\hline

        AriaNN  &Inter-party      &2.816  &  - &38.54      &55.04     &121.6      &-      &1161    &18944\\\hline
        \multirow{2}{*}{\scheme}    &Inter-party    &0.2058	&0.8371	&5.328	&7.931	&12.31	    &19.21 &187.7	&2106	\\\cline{2-10}
        &\LTH-CPU &0.4585	    &0.7958	    &7.235&10.24	&18.53	&2.270   &202.5	&3044	

        \\\hline
    
    \end{tabular}


    
    \label{tab:comm_sem}
    % \vspace*{-6mm}
\end{table*}

==> table4.tex <==
\begin{table*}[ht]
\small 
\renewcommand\arraystretch{1}
    \centering
    \caption{Inference communication (MB) of a 128 batch in a malicious setting.}
    \begin{tabular}{cc|cccccccc}
    \hline
    
        \multicolumn{2}{c|}{Framework} &  Network-A    &Network-B  &Network-C  &LeNet  &AlexNet    &Transformer    &VGG16 &ResNet18 \\\hline
        
        Falcon+     &Inter-party    &10.51     &41.33     &423.4&620.1    &1135    &340.0    &11543&139287\\\hline
        \multirow{2}{*}{\scheme}    &Inter-party        &0.8443     &2.0704	    &21.02&28.80    &48.68	&131.2     &838.6	&7500	\\
    \cline{2-10}
        &\LTH-CPU &1.070	&1.856	&16.88	&23.90	&43.23&5.296	&472.5	&7103


        \\\hline
    
    \end{tabular}


    
    \label{tab:comm_mal}
    % \vspace*{-6mm}
\end{table*}

==> table5.tex <==
\begin{table*}[ht]
\small 
% \renewcommand\arraystretch{1.2}
\setlength\tabcolsep{3pt}
    \centering
    \caption{Inference time (s) breakdown of a 128 batch in a semi-honest WAN/GPU setting, comparing with Falcon+.}
    \begin{tabular}{x{1.5cm}x{1.8cm}|x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.7cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.7cm}x{0.7cm}x{0.65cm}x{0.65cm}x{0.65cm}x{0.65cm}}
    \hline
        \multirow{2}{*}{Framework}&  \multirow{2}{*}{Component}&  \multicolumn{2}{c}{Network-A}    &\multicolumn{2}{c}{Network-B} &\multicolumn{2}{c}{Network-C}  &\multicolumn{2}{c}{LeNet} &\multicolumn{2}{c}{AlexNet}   &\multicolumn{2}{c}{Transformer}    &\multicolumn{2}{c}{VGG16}     &\multicolumn{2}{c}{ResNet18} \\
        && Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio& Time &Ratio\\ \hline
        \multirow{3}{*}{\scheme} &CPU/GPU &0.04  & 17\%  & 0.06  & 23\%  & 0.19  & 19\%  & 0.28  & 21\%  & 0.29  & 12\%  & 0.30  & 6\%  & 12.8  & 43\%  & 98.0 & 28\%  \\ 
       & Comm. &0.18  & 70\%  & 0.16  & 58\%  & 0.35  & 34\%  & 0.35  & 27\%  & 0.94  & 38\%  & 4.56  & 91\%  & 3.34  & 11\%  & 44.0 & 13\%  \\ 
       & LTH &0.03  & 13\%  & 0.05  & 19\%  & 0.48  & 47\%  & 0.68  & 52\%  & 1.24  & 50\%  & 0.16  & 3\%  & 13.8  & 46\%  & 207 & 59\%  \\ \hline
        \multirow{2}{*}{Falcon+} &CPU/GPU &0.08  & 6\%  & 0.20  & 14\%  & 1.80  & 25\%  & 2.50  & 28\%  & 4.09  & 11\%  & 3.95  & 1\%  & 47.6  & 39\%  & 523 & 36\%  \\ 
        &Comm. &1.40  & 94\%  & 1.27  & 86\%  & 5.52  & 75\%  & 6.37  & 72\%  & 34.4  & 89\%  & 317  & 99\%  & 74.4  & 61\%  & 916 & 64\%  \\\hline
    \end{tabular}
	

    
    
    \label{tab:breakdown}
    % \vspace*{-6mm}
\end{table*}
